A Distributed System-level Diagnosis Model for the Implementation of Unreliable Failure Detectors

Reliable systems require effective monitoring techniques for fault identification. System-level diagnosis was originally proposed in the 1960s as a test-based approach to monitor and identify faulty components of a general system. Over the last decades, several diagnosis models and strategies have been proposed, based on different fault models, and applied to the most diverse types of computer systems. In the 1990s, unreliable failure detectors emerged as an abstraction to enable consensus in asynchronous systems subject to crash faults. Since then, failure detectors have become the \textit{de facto} standard for monitoring distributed systems. The purpose of the present work is to fill a conceptual gap by presenting a distributed diagnosis model that is consistent with unreliable failure detectors. Results are presented for the number of tests/monitoring messages required, latency for event detection, as well as completeness and accuracy. Three different failure detectors compliant with the proposed model are presented, including vRing and vCube which provide scalable alternatives to the traditional all-monitor-all strategy adopted by most existing failure detectors.

==> Reviews.tex <==
NFV-SDN:

# Reviewer 1

This approach is very costly in terms of memory, storage, computation, and latency, however, the evaluation is focused on availability with various levels of redundancy.

While the problem addressed (highly available stateful VNFs) is an important one, the paper only presents a brute-force solution. Thus the technical contribution is limited and very likely the scheme is impractical due to various overheads. This may still have some academic value but a superficial reading of the paper gives an impression that this is a workable solution when in very likelihood the approach is prohibitively costly (discussed below) though the evaluation does not cover these overhead costs.

The experiment and evaluation section glosses over essential details such as checkpointing frequency and does not cover important metrics.

The overhead of the scheme in terms of extra memory (for hold/release Rx/Tx buffers), latency, computing and storage for VNF checkpoints is not discussed in evaluation.

Not very clear how the architecture accommodates redundant or load-balanced VNFs

The assumption that buffers and SFFs do not fail is not very realistic. Where are the buffers stored? Isn’t SFF either part of the VNF or another VNF/VNFC? Instead of claiming that this is a realistic assumption, it could be considered a separate problem to be tackled later.

Giving details of experiments is essential. Several questions are left unanswered, for example:
  - how many SFs in the SFC
  - is there one VNF per SF or is there redundancy/load balancing
  - if the VNFs are stateful then what is considered a full recovery?
  - is the functionality monitored - e.g. IDS/IPS letting through attack traffic
  - how often are the checkpoints taken

The checkpoint frequency is an essential parameter of the proposed scheme. But the experiment and evaluation section barely mentions this and the results are provided without specifying the checkpoint frequency.

The overhead of the scheme in terms of extra memory (for hold/release Rx/Tx buffers), latency for flows due to hold/release and checkpointing, computing and storage for VNF checkpoints, etc. are essential metrics for evaluation. The fact that Active-Active is better than Active-Standby or multiple replicas are better than zero or one replica is not surprising.

# Reviewer 2

The paper does not apply to widely used NFV MANO frameworks and is limited to docker containers.

The paper attempts to tackle an important issue in NFV orchestration, but its limited vision in no widely used MANO frameworks such as OSM, do not contribute to its overall pros. It is based on real-like experiments but as they are presented they seem to be more simulations than real testbed measurements.

# Reviewer 3

After recovering the status of a VNF a request is sent to NFV-MANO to update "the required information". Could you give more details on this. In a network service composed of many VNFs: if one of them crashes and is then replaced, how mano handles the inter-connectivity with the other VNFs?

What are the real benefits of the MR-AA case since a VNF is always replaced by only one replica?

Fig.4 should be better explained. I would have expected more comments on the throughput and packet loss during the recovery time.

Also could the author give more details on the tradeoff between the SFC availability and the impact of the resiliency mechanisms?

A more sophisticated baseline would be more interesting since it is expected that "any" recovery mechanism would enhance the performance.

In the related work section, Remus [7] seems to be very similar to the proposed approach. A further description that shows the similarities/differences between the two works would be interesting.

In the experimental evaluation, an assessment of the overhead introduced by the approach is expected: additional exchanged messages, overhead of the buffers on the memory, overhead of the checkpoints VNFs, etc..

IEEE Computing:

This paper only makes experiments to compare the differences between four different elastic mechanisms in NHAM. The paper lacks comparative experiments with other techniques and ablation experiments, which makes the paper lose its persuasion. This is clearly unsatisfactory.

The first line of the penultimate paragraph of section 2.1 of this paper, " NFV-MANO itself is organized in three main modules", the correct form of the phrase should be "organize into" instead of "organize in".


==> Sections/lix.tex <==

Processes are organized on a virtual hiearchical topology, the VCube.  When all processes are correct, the VCube is a hypercube. Processes of a  $d$-dimensional hypercube have identifiers consisting of $d$ bits. Two processes are virtually connected whenever their binary addresses differ by only 1 bit. 
The major advantage of the VCube is that as processes crash, the virtual topology  dynamically reorganizes itself, keeping multiple logarithmic properties.  

VCube~\cite{Duarte14} is a distributed diagnosis algorithm which organizes proceses in increasingly large clusters. A diagnosis algorithm is used to determine which processes in the system are faulty and which are not. %fault-free. 
The virtual edges of a VCube correspond to tests that correct processes execute on each other. VCube allows processes to obtain diagnostic information from any process tested correct. %employs timestamp on each message 
Diagnostic information is timestamped to allow processes to distinguish recent events. A tester process $i$ executes tests on a cluster $c_{i,s}$ of processes of size  $2^{s-1}$, such that $s = 1 ... \log_2 n $. Function $C_{i,s}$ (Equation \ref{equa:cis}) returns the ordered list of processes of each cluster: 

\begin{equation}
\label{equa:cis}
\mathlarger{c_{i,s} = \{ i \oplus 2^{s-1},\ _{c_{i \oplus 2^{s-1}},\ 1} , ...\ ,\ _{c_{i \oplus 2^{s-1}}, s-1} \}}
\end{equation}

where $\oplus$ is the bitwise exclusive or operator (\textit{xor}). Table \ref{table:vcube-membros} shows the $c_{i,s}$ function for 8 processes. In order to determine the edges of the virtual topology, for each node $i$, there is an edge $(j,i)$, such that $j$ is the first fault-free node in $c_{i,s}$, $s = 1 ... \log_2 n $. After a process detects that any other process has crashed, the set of edges (tests) is recomputed. For instance, in the example shown in Figure \ref{fig:topo-fault-p4}, process $p_4$ originally tests process $p_0$, but after it has crashed, the tester of process $p_0$ in the cluster with $s=3$ is $p_5$.

\begin{figure}[!ht]
	\centering
	
	\includegraphics[width=0.6\linewidth]{figures/vcube-fault-p4.pdf}
	\caption{Clusters of a VCube with dimension $d=3$.}
	\label{fig:topo-fault-p4}
\end{figure}


